Language of Bargaining

Leveraging an established exercise in negotiation education, we build a novel dataset for studying how the use of language shapes bilateral bargaining. Our dataset extends existing work in two ways: 1) we recruit participants via behavioral labs instead of crowdsourcing platforms and allow participants to negotiate through audio, enabling more naturalistic interactions; 2) we add a control setting where participants negotiate only through alternating, written numeric offers. Despite the two contrasting forms of communication, we find that the average agreed prices of the two treatments are identical. But when subjects can talk, fewer offers are exchanged, negotiations finish faster, the likelihood of reaching agreement rises, and the variance of prices at which subjects agree drops substantially. We further propose a taxonomy of speech acts in negotiation and enrich the dataset with annotated speech acts. Our work also reveals linguistic signals that are predictive of negotiation outcomes.

==> hypotheses.tex <==

\section{Hypotheses and Features}




\chenhao{Explain the testing framework}

In this section, we start by comparing speech between buyers and sellers based on their negotiation outcome.
Specifically, we consider four pairs of groups: 
\begin{itemize}
  \item Winning sellers vs losing sellers
  \item Winning buyers vs losing buyers 
  \item Winning buyers vs losing sellers
  \item Winning sellers vs losing buyers
\end{itemize}
For each proposed feature, we use a $t$-test to measure whether there is a statistically significant difference in the presence of that feature within each each group for each pair we consider. The basic unit in each group is one negotiation. We use the following notation to indicate statistical significance:

\begin{table}[ht!]
    \center
    \begin{tabular}{cc}
    {} & {} \\
    \toprule
    $p<1e-20$ & $\uparrow \uparrow \uparrow \uparrow  / \downarrow \downarrow \downarrow \downarrow$ \\
    $p<0.001$ & $\uparrow \uparrow \uparrow  / \downarrow \downarrow \downarrow $\\
    $p<0.01$ & $\uparrow \uparrow  / \downarrow \downarrow$ \\
    $p<0.05$ & $\uparrow  / \downarrow $ \\
    $p\geq0.05$ & $ -  / - $ \\
    \bottomrule
    \end{tabular}
\end{table}



\subsection{Lexical Features}

We consider categories in LIWC and hedging.


\chenhao{this can probably go to appendix}
\paragraph{LIWC.} Our lexical analysis framework considers psychometric markers in the buyer and seller's speech. We use the LIWC2015 lexicon of regular expressions and corresponding categories. The LIWC lexicon includes categories related to syntactic features as well as semantic ones. 

We present in Table \ref{tab:liwc} the statistically significant LIWC categories whose prevalence differs in buyers or sellers speech depending on whether they win or lose. The findings suggest that buyers who refer more often to themselves and, perhaps, their needs, requirements, or constraints are more successful. On the other hand, sellers who use the 2nd person pronoun "you" frequently appear to lose more often. One explanation is that this reveals deference to the buyer and their concerns. Perhaps it also belies a desperation to make the sale, where use of the word ``you'' suggests the seller wants find a compromise that satisfies the buyer. Losing buyers refer to cause and effects more often than those that win. Excessive justification or explanations of an offer or concern may be ineffective, conveying a weak position.

Notably, sellers who lose are far more likely to use affect-related language. Appeals to emotion are ineffective as a selling strategy. This supports the hypothesis that sellers who do not show their hand, or express emotional buy-in are more effective. Use of the first person singular pronoun ``I'' emphasises the speakers personal needs, emotions, desires, and consideration. We observe that this type of language is highly effective when buyers use it, rather than sellers. The speech of winning buyers contains more uses of the pronoun ``I'' than buyers who lose as well as sellers who lose. Furthermore, this strategy does not appear to be effective for sellers, as sellers that win use ``I'' less frequently than winning buyers.

On the other hand, we observe a clear relationship between explicit mention of the house and related vocabulary by the seller and success. Sellers who focus their position on and speak about the house itself and accompanying features more than the buyer have an advantage. In contrast, mentions of leisure produce an asymmetric advantage in favor of the buyer. This may suggest that preferences around leisure are more subjective, and thus, puts the seller in a weaker position for making a case for against the location or amenities of the house being sold. This is different from the universally accepted signals of value associated with the features of a house. For example, whether a home is near a park or the downtown of a city are less universally appreciated features.
\chenhao{these few paragraphs are good, maybe add a paragraph header for each one. I am not sure how these relate to later texts?}

\begin{table*}[ht!]
    \centering
    \small
    \input{./tables/liwc.tex}
    \caption{LIWC}
    \label{tab:liwc}
\end{table*}

\paragraph{Hedging.} Words that reflect uncertainty, equivocation, or a lack of confidence are considered \textit{hedges}. We measure the prevalence of these terms in the speech of buyers and sellers using a lexicon of 255 regular expressions. We correlate these statistics with bargaining outcomes. 

There is no significant difference in hedging between sellers and buyers that win or lose. However, sellers tend to use hedges more than buyers, especially as negotiations increase in length. \mourad{add data} 
\chenhao{we can drop this if we do not have more interesting things to say}

\subsection{Negotiation Acts}


\subsection{Exploratory Analysis}
Finally, we use Fightin' words to understand the differences between different groups in an exploratory fashion. 
\chenhao{maybe we should have other groups}

As one of the lexical analyses of the language used in the \textit{natural language} treatment, we compare the seller and buyer's use of \textit{Fightin' Words}. We further investigate how the use of \textit{Fightin' Words} change depending on the outcome of the negotiations.
\chenhao{fightin' words go later?}

\begin{table*}[t!]
    \begin{subtable}[h]{\textwidth}
        \caption{Differences Within Roles Across Outcomes}
        \label{tab:fw_same}
        \let\center\empty
        \let\endcenter\relax
        \centering
        \resizebox{1\textwidth}{!}{\input{./tables/fightin_words/same_win_lose_adv_fighting.tex}}
    \end{subtable}

    \begin{subtable}[h]{\textwidth}
        \caption{Differences Across Roles and Outcomes}
        \label{tab:fw_dif}
        \let\center\empty
        \let\endcenter\relax
        \centering
        \resizebox{1\textwidth}{!}{\input{./tables/fightin_words/dif_win_lose_adv_fighting.tex}}
    \end{subtable}
    \caption{Fightin' Words: The table reports statistically significant deviations from mean usage of certain ngrams. The significance of each ngram is indicated by its z-score. Table \ref{tab:fw_same} compares lexicons between winners and losers of the same role. Table \ref{tab:fw_dif} compares lexicons between winners and losers of opposing roles.}
    \label{tab:fw}
\end{table*}

Notably, sellers' use of the term ``home'' is correlated with losing whereas saying ``my house'' is correlated with winning. We hypothesize that this difference is due to ``home'' revealing a greater sense of personal connection and investment in the house being sold, which puts the seller in a weaker position of negotiation, as they may be more emotionally invested. Other differences between the seller winning and losing are reflected by an increased use of the 2nd person pronoun, ``you'' rather than ``we'' and mentions related to the size of the house.

\textbf{Comparison Works.} Table \ref{tab:fw_dif} presents differences in speech patterns between winners and losers of opposing roles. Winning buyers refer more often to other considerations and properties, forcing comparison. Sellers are put at a disadvantage when they allow the buyer to prompt them in justifying their pricing relative to other similar properties. This puts sellers at a disadvantage, as long as they cannot perfectly justify the differences, which is unlikely. Interestingly, in this scenario, sellers appear to fall back on highlighting less tangible features of the house being sold, mentioning that its ``new decorated.''

In the complimentary comparison, sellers who win highlight features of their home that may be more difficult to strictly compare with other properties. These ngrams, like ``beautiful'', ``fireplace'', ``bedroom'', and ``space'', are more qualitative and evocative than listing numerical facts like square footage. 

\subsection{Feature Engineering}
\chenhao{what is this section doing?}
\subsubsection{Outcome}

In our regression experiments, we control for the number of buyer and seller tokens which allows us to study the marginal effects of negotiation actions by each party on the final agreed price. We observe that an increase in \textbf{buyer repeat offers} tends to drive down the final price. Similarly, \textbf{buyer pushes} also drive down the final price. These findings support the hypothesis that, for buyers, being more assertive and aggressive in negotiation is an advantageous strategy.

\subsubsection{Duration}
We conduct a similar analysis using negotiation duration as the outcome variable. We observe that a one unit increase in \textbf{seller new offers} increases the duration of the conversation by 4 minutes, on average. One additional \textbf{buyer push} increases the duration by approximately 1.5 minutes. These results would suggest that seller new offers and buyer pushes have a strong affect on complicating negotiations, resulting in longer convergence times.


\subsection{Lexical}
Using LIWC analysis, we observe that buyers tend to use far more comparison words in general and, especially when they win. Buyers also use more differentiation words 3x more (e.g., ``but'', ``not'', ``if'', ``or'') when they win than when they lose.

The proportion of seller tokens related to reward is higher when they win (approx. 2x). Relatedly, words related to risk are only employed in the context of buyer wins.

Discrepancy-related word usage is highest in buyer speech when they win (2x higher than when they lose). 

Use of tentative words (``if'', ``or'', ``any'', ``something'') is highest for both seller and buyer when they win. This may provide some evidence for politeness being an effective strategy.

Certainty is most common in seller speech when they lose. This may suggest that presenting too rigid of a stance creates an adversarial relationship between the seller and buyer resulting in more aggressive negotiations from the buyer.

When the seller loses, they use the 2nd person pronoun ``you'' 5x less than in any another setting, perhaps suggesting that not being explicit towards and considerate of the other participant (the buyer) is indicative of ineffective strategy.

Positive emotions words (``good'', ``love'', ``happy'', ``hope'') are more common in seller and buyer speech when they lose. It may be that expressing positive emotion is ineffective for eliciting empathy, compassion or even pity from the other person, thus making them less likely to be willing to negotiate.

The proportion of buyer speech related to money is over 2x as high when they win than when they lose. This may support the hypothesis that buyers are more successful when assertive and talk about their personal financial constraints.

drives
differentiation (differ)
comparison words (compare)


==> tables/fightin_words/dif_win_lose_adv_fighting.tex <==
\begin{tabular}{  m{0.5\linewidth}  m{0.5\linewidth} } 
\toprule
  \textbf{Buyer Win $\rightarrow$ Seller Lose} &\textbf{ Seller Win $\rightarrow$ Buyer Lose} \\
\midrule
more (5.311), around (4.97), looking at (4.558), 30 (4.267), looking (4.094), similar (3.863), 230 (3.813), range (3.782), to make (3.782), like (3.779), some (3.77), if we (3.614), square feet (3.549), to 30 (3.524), high (3.514), you see (-3.016), everything (-3.056), newly decorated (-3.056), anything (-3.056), think it (-3.059), we have (-3.095), park (-3.105), the house (-3.112), think (-3.21), newly (-3.294), it (-3.601), house (-3.737), decorated (-3.747), been (-3.791), you (-6.745) & sell (5.564), low (5.026), space (4.304), to sell (4.174), my house (3.812), has (3.792), beautiful (3.722), master (3.722), since (3.701), fireplaces (3.672), bedroom (3.621), four (3.584), if you (3.58), pretty (3.574), already (3.565), your (-3.246), high (-3.284), 213 (-3.287), could (-3.321), 220 (-3.347), your house (-3.538), right (-3.813), like you know (-3.839), still (-3.931), something (-4.053), me (-4.118), looking (-4.159), looking at (-4.172), budget (-4.585), like (-4.981) \\
\bottomrule
\end{tabular}


==> tables/fightin_words/same_win_lose_adv_fighting.tex <==
\begin{tabular}{  m{0.5\linewidth}  m{0.5\linewidth} } 
\toprule 
\textbf{Seller Win $\rightarrow$ Seller Lose} & \textbf{Buyer Win $\rightarrow$ Buyer Lose} \\
\midrule
25 (4.067), we (3.976), square feet (3.933), 230 (3.882), feet (3.83), space (3.592), sell (3.543), less than (3.43), 230 000 (3.358), if we (3.315), low (3.293), my house (2.806), 225 (2.78), mm (2.768), 500 (2.742), stuff (-2.849), you re (-2.889), home (-3.0), appreciate (-3.102), it really (-3.174), did (-3.196), you see (-3.322), this (-3.358), to 35 (-3.666), get (-3.696), uh (-3.771), 32 (-4.003), 40 (-4.233), 35 (-4.961), you (-5.919) & 30 (5.156), um (4.01), 35 (3.801), to 30 (3.73), 33 (3.667), 31 (3.315), more (3.296), 230 (3.223), beautiful (3.181), yeah (3.101), 32 (3.075), thinking (2.99), if you can (2.832), all the (2.829), if you (2.821), 500 (-2.7), feel (-2.764), anything (-2.841), something (-2.894), house and (-2.958), 225 (-3.175), the house (-3.321), 25 (-3.379), you know like (-3.465), know like (-3.484), like you know (-3.698), house (-3.701), 28 (-3.828), 200 (-3.895), like you (-4.099) \\
\bottomrule
\end{tabular}


==> tables/liwc.tex <==
\begin{tabular}{lllll}
\toprule
{} & Seller Win / Seller Lose & Buyer Win / Buyer Lose &                 Buyer Win / Seller Lose &                 Seller Win / Buyer Lose \\
\midrule
achiev       &              (-0.6, 0.5) &             (0.1, 0.9) &                             (-0.4, 0.7) &                             (-0.2, 0.8) \\
adj          &               (1.3, 0.2) &             (0.6, 0.6) &                              (0.8, 0.4) &                              (1.1, 0.3) \\
adverb       &              (-0.6, 0.5) &            (-0.1, 0.9) &                             (-0.1, 0.9) &                             (-0.6, 0.6) \\
affect       &              (-0.2, 0.9) &            (-1.5, 0.1) &               $\downarrow$ $\downarrow$ &                              (1.2, 0.2) \\
affiliation  &               (1.9, 0.1) &            (-0.8, 0.5) &                              (0.0, 1.0) &                              (1.3, 0.2) \\
anger        &               (0.5, 0.6) &             (1.0, 0.3) &                              (1.1, 0.3) &                              (0.5, 0.6) \\
anx          &              (-0.1, 0.9) &             (1.0, 0.3) &                              (1.0, 0.3) &                             (-0.2, 0.8) \\
article      &               (0.6, 0.6) &            (-0.9, 0.4) &                             (-0.5, 0.6) &                              (0.3, 0.8) \\
assent       &              (-1.1, 0.3) &             (0.9, 0.4) &                              (1.4, 0.2) &                             (-1.1, 0.3) \\
auxverb      &              (-0.1, 1.0) &            (-0.9, 0.4) &                             (-0.0, 1.0) &                             (-1.0, 0.3) \\
bio          &               (1.1, 0.3) &             (0.6, 0.5) &                             (-0.5, 0.6) &                              $\uparrow$ \\
body         &               $\uparrow$ &             (0.1, 0.9) &                              (1.6, 0.1) &                              (0.3, 0.7) \\
cause        &              (-1.3, 0.2) &           $\downarrow$ &                             (-1.4, 0.2) &                             (-1.9, 0.1) \\
certain      &             $\downarrow$ &            (-0.2, 0.8) &               $\downarrow$ $\downarrow$ &                              (0.6, 0.5) \\
cogproc      &              (-1.4, 0.2) &            (-1.0, 0.3) &                             (-1.0, 0.3) &                             (-1.4, 0.2) \\
compare      &               (0.8, 0.4) &             (0.1, 1.0) &                              (1.8, 0.1) &                             (-0.9, 0.4) \\
conj         &              (-1.8, 0.1) &            (-1.8, 0.1) &               $\downarrow$ $\downarrow$ &                             (-0.8, 0.4) \\
death        &                        - &            (-0.2, 0.9) &                                       - &                             (-0.7, 0.5) \\
differ       &              (-1.0, 0.3) &             (0.4, 0.7) &                             (-0.6, 0.6) &                             (-0.1, 1.0) \\
discrep      &              (-0.3, 0.8) &            (-0.2, 0.9) &                              (0.5, 0.6) &                             (-1.0, 0.3) \\
drives       &               (1.8, 0.1) &            (-1.0, 0.3) &                             (-0.3, 0.8) &                              (1.3, 0.2) \\
family       &               (0.4, 0.7) &            (-0.5, 0.6) &                              (0.0, 1.0) &                             (-0.2, 0.8) \\
feel         &              (-0.7, 0.5) &           $\downarrow$ &                             (-1.7, 0.1) &                             (-1.5, 0.1) \\
female       &               $\uparrow$ &            (-1.6, 0.1) &                              (1.5, 0.1) &                             (-1.0, 0.3) \\
filler       &               (1.6, 0.1) &             (0.5, 0.6) &                              (1.5, 0.1) &                              (0.1, 0.9) \\
focusfuture  &              (-0.1, 0.9) &             (0.3, 0.8) &                              (0.0, 1.0) &                              (0.2, 0.9) \\
focuspast    &              (-0.4, 0.7) &            (-0.7, 0.5) &               $\downarrow$ $\downarrow$ &                              (1.6, 0.1) \\
focuspresent &               (0.3, 0.7) &            (-0.8, 0.4) &                             (-0.1, 0.9) &                             (-0.4, 0.7) \\
friend       &              (-0.2, 0.9) &            (-0.3, 0.7) &                             (-0.1, 0.9) &                             (-0.4, 0.7) \\
function     &              (-0.8, 0.4) &            (-1.2, 0.3) &                             (-0.8, 0.4) &                             (-1.1, 0.3) \\
health       &              (-0.8, 0.4) &             (1.8, 0.1) &                             (-0.9, 0.4) &                              $\uparrow$ \\
hear         &               (0.5, 0.6) &            (-0.2, 0.9) &                             (-0.3, 0.8) &                              (0.5, 0.6) \\
home         &               (1.4, 0.2) &            (-1.5, 0.1) &               $\downarrow$ $\downarrow$ &                   $\uparrow$ $\uparrow$ \\
i            &              (-0.9, 0.4) &             $\uparrow$ &        $\uparrow$ $\uparrow$ $\uparrow$ &                            $\downarrow$ \\
informal     &              (-0.0, 1.0) &             (1.7, 0.1) &                              $\uparrow$ &                             (-0.2, 0.9) \\
ingest       &              (-0.1, 0.9) &            (-0.2, 0.9) &               $\downarrow$ $\downarrow$ &                   $\uparrow$ $\uparrow$ \\
insight      &              (-0.9, 0.4) &            (-0.5, 0.6) &                             (-0.4, 0.7) &                             (-0.9, 0.4) \\
interrog     &              (-0.3, 0.8) &             (0.1, 0.9) &                             (-0.4, 0.7) &                              (0.2, 0.8) \\
ipron        &              (-0.1, 1.0) &            (-0.6, 0.6) &                             (-0.9, 0.4) &                              (0.3, 0.7) \\
leisure      &               (0.5, 0.6) &            (-0.9, 0.4) &  $\downarrow$ $\downarrow$ $\downarrow$ &                   $\uparrow$ $\uparrow$ \\
male         &              (-1.6, 0.1) &            (-0.9, 0.4) &                             (-1.3, 0.2) &                             (-1.1, 0.3) \\
money        &               (0.4, 0.7) &            (-0.6, 0.5) &                              (1.3, 0.2) &                             (-1.6, 0.1) \\
motion       &               (1.6, 0.1) &             (0.4, 0.7) &                              (0.3, 0.8) &                              (1.5, 0.1) \\
negate       &               (0.2, 0.9) &            (-0.5, 0.6) &                             (-1.1, 0.3) &                              (0.8, 0.4) \\
negemo       &               (0.5, 0.6) &             (0.2, 0.8) &                            $\downarrow$ &        $\uparrow$ $\uparrow$ $\uparrow$ \\
netspeak     &               (0.2, 0.8) &             (1.1, 0.3) &                              (2.0, 0.1) &                             (-0.7, 0.5) \\
nonflu       &               (0.8, 0.4) &             (1.8, 0.1) &                              (1.9, 0.1) &                              (0.8, 0.4) \\
number       &               (1.2, 0.2) &             $\uparrow$ &                              (0.8, 0.4) &                              $\uparrow$ \\
percept      &               (0.2, 0.9) &            (-1.0, 0.3) &                              (1.1, 0.3) &                             (-1.8, 0.1) \\
posemo       &              (-0.5, 0.6) &            (-1.6, 0.1) &                            $\downarrow$ &                              (0.3, 0.8) \\
power        &               (1.8, 0.1) &             (0.4, 0.7) &                              (1.0, 0.3) &                              (1.2, 0.2) \\
ppron        &              (-1.0, 0.3) &             (1.2, 0.2) &                              (1.2, 0.2) &                             (-1.2, 0.2) \\
prep         &               (0.7, 0.5) &            (-1.0, 0.3) &                              (0.5, 0.6) &                             (-1.0, 0.3) \\
pronoun      &              (-0.8, 0.4) &             (0.5, 0.6) &                              (0.4, 0.7) &                             (-0.8, 0.4) \\
quant        &               (1.8, 0.1) &             (0.9, 0.4) &                              $\uparrow$ &                              (0.3, 0.7) \\
relativ      &               $\uparrow$ &             (0.4, 0.7) &                             (-0.2, 0.8) &                              $\uparrow$ \\
relig        &               (0.8, 0.5) &             (0.4, 0.7) &                              (0.8, 0.5) &                              (0.4, 0.7) \\
reward       &              (-0.7, 0.5) &            (-1.9, 0.1) &               $\downarrow$ $\downarrow$ &                              (0.3, 0.8) \\
risk         &               (0.4, 0.7) &            (-0.7, 0.5) &                              (0.5, 0.6) &                             (-1.0, 0.3) \\
sad          &               (0.7, 0.5) &            (-0.7, 0.5) &  $\downarrow$ $\downarrow$ $\downarrow$ &        $\uparrow$ $\uparrow$ $\uparrow$ \\
see          &               (0.3, 0.8) &             (0.2, 0.9) &                              $\uparrow$ &                             (-2.0, 0.1) \\
sexual       &               (0.3, 0.8) &            (-0.5, 0.6) &                              (0.3, 0.8) &                             (-0.5, 0.6) \\
shehe        &               (1.1, 0.3) &            (-1.3, 0.2) &                              (0.4, 0.7) &                             (-0.7, 0.5) \\
social       &              (-0.2, 0.8) &            (-1.1, 0.3) &                             (-1.9, 0.1) &                              (0.9, 0.4) \\
space        &               (1.4, 0.2) &             (0.7, 0.5) &                              (0.4, 0.7) &                              (1.7, 0.1) \\
swear        &               (0.4, 0.7) &             (1.2, 0.2) &                              (0.7, 0.5) &                              (1.0, 0.3) \\
tentat       &               (0.9, 0.3) &             (0.7, 0.5) &                              (0.9, 0.4) &                              (0.7, 0.5) \\
they         &              (-0.3, 0.8) &             (0.8, 0.4) &                              (0.9, 0.4) &                             (-0.4, 0.7) \\
time         &               (0.9, 0.4) &            (-0.4, 0.7) &                             (-1.1, 0.3) &                              (1.7, 0.1) \\
verb         &               (0.0, 1.0) &            (-0.9, 0.4) &                             (-0.0, 1.0) &                             (-0.8, 0.4) \\
we           &               $\uparrow$ &            (-0.9, 0.4) &                             (-0.5, 0.6) &                              (1.8, 0.1) \\
work         &              (-0.8, 0.4) &            (-1.4, 0.2) &                              (1.5, 0.1) &  $\downarrow$ $\downarrow$ $\downarrow$ \\
you          &              (-1.9, 0.1) &            (-0.7, 0.5) &                            $\downarrow$ &                             (-0.1, 0.9) \\
\bottomrule
\end{tabular}

